A Tighter Upper Bound for the Number of Distinct Squares in Circular Words

A \emph{square} is a word of the form $uu$, where $u$ is a nonempty finite word. Given a finite word $w$ of length $n$, let $[w]$ denote the corresponding \emph{circular word}, i.e., the set of all cyclic rotations of $w$. We study the number of distinct square factors of the elements of $[w]$. Amit and Gawrychowski first showed that this number is upper bounded by $3.14n$. In a recent article, Charalampopoulos et al. improved this upper bound to $1.8n$ and conjectured that the sharp upper bound is $1.5n$. In this note, we improve this upper bound to $\frac{5}{3}n$.

==> Biblio.tex <==
\newpage\noindent
{\bf Acknowledgements}. The last author is grateful to Gilbert Labelle for
putting him on the track of the thesis of P.K.  Stockmeyer.

\begin{thebibliography}{99}
\newcommand{\aut}[1]{{\sc #1}}

\bibitem{auger} P. Auger, Analyse d'\'equations combinatoires en th\'eorie des esp\`eces, Ph.D.,
Universit\'e du Qu\'ebec \`a Montr\'eal, Publications du LaCIM, Vol. 26 (2000)

\bibitem{labelle} P. Auger, G. Labelle, P. Leroux, Combinatorial additive formulas and applications,
{\em Advances in Applied Maths}, {\bf 28} (2002) 302--342.

\bibitem{abcd} J.P. Allouche, M. Baake, J. Cassaigne, D. Damanik,
Palindrome complexity, {\em Theoret. Comput. Sci.}, {\bf 292} (2003) 9--31. 

\bibitem{bl} S. Brlek, A. Ladouceur, A note on differentiable palindromes,
{\em Theoret. Comput. Sci.}, {\bf 302}/1-3 (2003) 167--178.

\bibitem{dp} X. Droubay, G. Pirillo, Palindromes and Sturmian words, 
{\em Theoret. Comput. Sci.}, {\bf 223} (1999) 73--85.

\bibitem{djp} X. Droubay, J. Justin, G. Pirillo, Episturmian words and some constructions of de Luca and Rauzy,
{\em Theoret. Comput. Sci.}, {\bf 255} (2001) 539--553.

\bibitem{humphreys} J.E. Humphreys, Introduction to Lie algebras and representation theory, Springer Verlag (1980).


\bibitem{lothaire1} M. Lothaire, Combinatorics on words, 
Addison-Wesley, 1983. 

\bibitem{lothaire} M. Lothaire, Algebraic Combinatorics on words, 
Cambridge University Press, 2002. 

\bibitem{deLu}
A. de Luca, Sturmian words: structure, combinatorics, and their arithmetics,
{\em Theoret. Comput. Sci.}, {\bf 183} (1997) 45--82.

\bibitem{mo} M. Morse and G. Hedlund, Symbolic Dynamics, 
{\em Amer. J. Math.}, {\bf 60} (1938) 815--866.


\bibitem{stock} P. K. Stockmeyer, Enumeration of graphs with prescribed automorphism group, {\it Ph. D. thesis}, University of Michigan (1971). 





\end{thebibliography}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "biblio"
%%% End: 


==> Concluding.tex <==
\section{Concluding Remarks}
\label{sec:concl}

The identity~\eqref{eq:squares} presented here for square factors is a natural extension of the Brlek-Reutenauer identity for palindromes and $\sigma$-palindromes.
Whether it holds for other patterns, is worth considering.
Indeed, the computation of lacunas of a certain type is easy to implement and the problem is to deal with multiplicities at each position.
In the case of $\sigma$-palindromes the multiplicity at each position is $1$, while in the case of squares it can be at most $2$ (the double squares of Fraenkel and Simpson).

Let us mention the case of overlaps, factors of the type $xuxux$~\cite{JamesNarad}, which contain squares, so that the overlap complexity is less than the square complexity.
An easy adaptation of the algorithm described in Section~\ref{sec:defect} allows to compute the lacunas, while multiplicity is easy to check. 
Patterns of the form $xx\widetilde{x}$, which contain a square overlapping a palindrome \cite{JamesNarad} also fall in our framework.

Moreover, the design of an efficient algorithm for determining the pattern complexity is, in general, an open problem. Nevertheless, in the case of palindromes and squares, there are linear algorithms for computing these patterns, by using suffix-trees~\cite{gus1}.
For some other patterns, the problem is open and begs for a systematic investigation. 

While it is proved that $S(w) \le \floor{11 / 6}|w|$, it is commonly believed that the square complexity of a word is bounded by the length of the same.
Deza and Franek proposed~\cite{DezaFranek15} the following conjecture (a stronger conjecture for binary alphabet is proposed in~\cite{JonoskaMS}).

\begin{conjecture}
\label{conj:sw}
 For every word $w \in A^\infty$, one has $S(w) \leq |w| - |\Alphabet(w)| + 1$.
\end{conjecture}

The bound in the previous conjecture is sharp.
Indeed every word $w$ having $|w|$ different letters (for instance, $\varepsilon$ or a letter $a \in A$) satisfies $S(w) = 1$.
Recently, Deza and Franek proved~\cite{DezaFranek17} that a similar inequality is verified for the number of runs in a word (a {\em run} is a maximal primitively rooted repetition with a possibly fractional exponent).
Note that Conjecture~\ref{conj:sw} would implies that $\D_s(w) \ge |\Alphabet(w)|$.
